Prototype Learning for Out-of-Distribution Polyp Segmentation

Existing polyp segmentation models from colonoscopy images often fail to provide reliable segmentation results on datasets from different centers, limiting their applicability. Our objective in this study is to create a robust and well-generalized segmentation model named PrototypeLab that can assist in polyp segmentation. To achieve this, we incorporate various lighting modes such as White light imaging (WLI), Blue light imaging (BLI), Linked color imaging (LCI), and Flexible spectral imaging color enhancement (FICE) into our new segmentation model, that learns to create prototypes for each class of object present in the images. These prototypes represent the characteristic features of the objects, such as their shape, texture, color. Our model is designed to perform effectively on out-of-distribution (OOD) datasets from multiple centers. We first generate a coarse mask that is used to learn prototypes for the main object class, which are then employed to generate the final segmentation mask. By using prototypes to represent the main class, our approach handles the variability present in the medical images and generalize well to new data since prototype capture the underlying distribution of the data. PrototypeLab offers a promising solution with a dice coefficient of $\geq$ 90\% and mIoU $\geq$ 85\% with a near real-time processing speed for polyp segmentation. It achieved superior performance on OOD datasets compared to 16 state-of-the-art image segmentation architectures, potentially improving clinical outcomes. Codes are available at https://github.com/xxxxx/PrototypeLab.

==> introduction-jr.tex <==
\section{Introduction}

Most gastrointestinal (GI) cancers are preventable. In 2018, the five major types of GI cancers, which include those of the stomach, liver, oesophagus, and colorectum account for 26\% of the global cancer incidence and 35\% of all cancer deaths~\cite{arnold2020global}. Endoscopy, a vital tool for screening and disease surveillance, is however heavily operator dependent and 12\% of cancers are missed~\cite{menon2014commonly}. Artificial intelligence-based systems can play a vital role in improving diagnostic quality. However, it is critical that these tools integrate directly into the existing clinical workflow and generalize well to the previously unseen data. 

Today, high-definition endoscopes provide a sufficient resolution to allow for a detailed visualisation of the mucosal surface. In addition to the conventional white light imaging (WLI) modality, autofluorescence imaging, and electronic chemoendoscopy techniques such as narrow-band imaging have been developed to improve the early detection of cancer and its precursors~\cite{subramanian2014advanced}. It is important that any computer assisted methods should work seamlessly in these different modalities and avoid the need for any modality-specific training. Developing such a modality agnostic approach for detection and segmentation of pre-cancerous changes in the esophagus, and polyps in the lower GI is the focus of this paper.  

\indent{Convolutional} Neural Network (CNN) based approaches~\cite{FCN,Olaf:MICCAI2015,10.1007/978-3-030-01234-2_49}, all  well established in biomedical imaging, have been applied to segmentation tasks in GI endoscopy ~\cite{ALI2021102002,guo2020polyp,wu2021elnet}. Wu et al.~\cite{wu2021elnet} proposed a dual neural network based on U-Net with ResNet backbone for automatic esophageal lesion segmentation. Guo et al.~\cite{guo2020polyp} utilized {a} FCN-based architecture with atrous kernels to segment polyps. However, all these supervised approaches are trained on WLI endoscopy and do not support working in different imaging modalities. 
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\textwidth]{imgs/Fig1.png}
\caption{Example images and masks of the two GI datasets for which source and target domains are separated based on their modality.~\label{fig:1}}
% The top row illustrates the Barrett's esophagus while the bottom row represents the polyps. Here, the left column correspond to white light imaging (WLI) modality which is source domain in our study and the right column demonstrate the narrow band imaging (NBI) modality used as target domain.
\end{figure}
%
To date, the problem of quantifying disease related changes in NBI, which can produce a very different appearance of the mucosal surface when compared to WLI (see Fig.~\ref{fig:1}) has not been addressed. Training methods for different imaging modalities independently is prohibitive. Firstly, extensive training datasets that cover a similar range of conditions would need to be curated to ensure a comparable performance. Secondly, manual annotations by human experts are required which is not only labour intensive but also expensive. 
%
To tackle these issues domain adaptation methods have been used to adapt trained models to unseen target data for segmentation~\cite{Tsai,CardioUDA,pmlr-v121-haq20a,10.1007/978-3-030-58539-6_25}. 
{Although these methods promise to generalise, so far there are only a few examples of applying such methods to medical data ~\cite{CardioUDA,pmlr-v121-haq20a}}. Additionally, the available methods still under-perform and have not been adapted for extremely diverse modality cases such as that in the GI endoscopy. 

%Tsai et al.~\cite{Tsai} developed a domain adaptation model for semantic segmentation based on a multi-level adversarial network that shares the segmentation loss for both source and target domains. In the discriminator network, target domain predictions are matched to the source domain predictions whether the input is from the source or target domain via an adversarial loss. In the context of biomedical image segmentation, Dong et al.~\cite{CardioUDA} proposed an unsupervised domain adaptation (UDA) technique for cardiothoracic ratio estimation by performing domain invariant chest organ segmentation. Haq et al.~\cite{pmlr-v121-haq20a} introduced an alternative UDA framework that included a decoder network to reconstruct the input images for cell segmentation. Pandey et al.~\cite{10.1007/978-3-030-58539-6_25} employed UDA approach to segment human skin under different imaging modalities via a variational auto-encoder (VAE) based generative model.
%

To develop a modality-agnostic approach, we propose to use an unsupervised domain adaptation (UDA) technique that can be trained on available single WLI modality dataset and can be applied on an unseen NBI imagery. For such settings, where classical supervised models fail to generalize and perform poorly, we show that our proposed target-independent UDA technique, EndoUDA, has the potential to generalize and {to} provide improved segmentation on NBI modality for both BE and polyp datasets. 
%


==> introduction-old.tex <==
Esophageal adenocarcinoma (EAC) is the seventh most common cause of cancer deaths with 14\% five years survival rate while colorectal cancer (CRC) has the third highest mortality rate with overall five-year survival rate of only around 68\%. One common early precursor of EAC is the Barrett's oesophagus (BE) in esophagus~\cite{cook2018cancer} and polyp in the CRC~\cite{holme2013flexible}. Changes in the surface color (e.g., changes in color of the mucosa in BE, see Fig.~\ref{fig:1} (top)) and the surface topology (e.g., protrusion of mucosa, see Fig.~\ref{fig:1} (bottom)) of the tissue and other irregularities indicate precancerous changes. Studies have shown that population-wide screening and quantification can advance the prognosis and can even reduce the incidences~\cite{holme2013flexible}. Endoscopy is the standard tool for both diagnostic and therapeutic procedures for reducing risks of such occurrences. It is thus imminently important to quantify these areas accurately and monitor these changes. While manual comparison of these areas is difficult to perform, automated segmentation methods can help in to obtain more accurate and measurable quantification of these areas. 

Today, there are many such methods built for segmentation of such areas but most of these methods require abundant amount of annotations. It is evident that manual segmentation of specialized medical conditions such as BE and polyp are prone to human subjectivity and require extensive knowledge in clinical endoscopy. Additionally, such processes are labor intensive due to the large annotation time required for pixel-wise delineation of such areas in these images. Due to the high risk associated with these cancer precursors, often complimentary modality such as narrow-band imaging (NBI) is widely used in addition to the conventional white-light imaging (WLI) modality. While, most automated methods for segmentation are based on the WLI modality, no work is done in direction of quantifying NBI modality which can produce a very diverse set of images as shown in Fig.~\ref{fig:1} compared to WLI. The lack of abundant and curated NBI dataset is a major bottleneck for applying supervised techniques. Additionally, curating modality specific dataset will require an additional enormous amount of time from clinical experts. To mitigate such problems, we propose to use unsupervised domain adaptation (UDA) technique that can be trained on available single WLI modality dataset and can be applied on an unseen NBI modality dataset. For such settings, where classical supervised models fail to generalize and perform poorly, we show that our proposed UDA technique has the potential to generalize and provide improved segmentation on NBI modality for both BE and polyp datasets. 

\indent{Convolutional} Neural Network (CNN) based approaches such as Fully Convolutional Network (FCN)~\cite{FCN}, U-Net~\cite{Olaf:MICCAI2015}, DeepLab~\cite{10.1007/978-3-030-01234-2_49} are known to perform well in the biomedical image segmentation domain, including segmentation tasks on gastrointestinal (GI) endoscopy~\cite{ALI2021102002,guo2020polyp,wu2021elnet,mendel2017barrett}. Wu et al.~\cite{wu2021elnet} proposed a dual neural network based on U-Net with ResNet backbone for automatic esophageal lesion segmentation. Similarly, majority of the teams in the multi-class GI disease segmentation challenge~\cite{ALI2021102002} also used U-Net-based models. Guo et al.~\cite{guo2020polyp} utilized FCN-based architecture with atrous kernels to segment polyps. All of these supervised methods are built on a single WLI modality endoscopy. However, in clinical endoscopy, endoscopists often use other complimentary modalities such as widely used NBI to characterize the tissue. Due to the incapability of these fully supervised models to generalize well to different imaging modalities due to domain shift, and lack of reliable and bulk annotations required by supervised models for each specific modality; there has not been much work done towards solving this problem in medical imaging domain. In this context, domain adaptation~\cite{ADDA} approaches have been proposed for unsupervised or semi-supervised domain learning wherein annotations are not required in the target (test) dataset consisting of a different imaging modality or dataset. 

Tsai et al.~\cite{Tsai} developed a domain adaptation model for semantic segmentation based on a multi-level adversarial network that shares the segmentation loss for both source and target domains. In the discriminator network, target domain predictions are matched to the source domain predictions whether the input is from the source or target domain via an adversarial loss. In the context of biomedical image segmentation, Dong et al.~\cite{CardioUDA} proposed an unsupervised domain adaptation (UDA) technique for cardiothoracic ratio estimation by performing domain invariant chest organ segmentation. Haq et al.~\cite{pmlr-v121-haq20a} introduced an alternative UDA framework that included a decoder network to reconstruct the input images for cell segmentation. Pandey et al.~\cite{10.1007/978-3-030-58539-6_25} employed UDA approach to segment human skin under different imaging modalities via a variational auto-encoder (VAE) based generative model. The existing GI endoscopy image segmentation methods are however limited by the fully supervised methods~\cite{ALI2021102002,guo2020polyp,wu2021elnet}. 

To the best of our knowledge, this is the first work that exploits the learned latent vector space representation in the VAE obtained from the source domain (WLI) to generalize to segment unseen target (NBI) dataset in GI endoscopy. Our novel EndoUDA utilizes a simplified architecture compared to the state-of-the-art GLSS method~\cite{10.1007/978-3-030-58539-6_25}. Our architecture includes the utilization of a common EfficientNet-B4 backbone for both U-Net and VAE encoder, and a weighted loss function for faster convergence of target latent space projection during inference. Our contributions can be summarised as follows: 1) Unsupervised domain adaptation approach (EndoUDA) based on generative model for the segmentation of GI endoscopy anomalies for unseen NBI modality, 2) simplified network with shared encoder for VAE and segmentation modules, 3) a weighted loss for achieving optimal nearest clone of target image during inference, 4) a comprehensive comparison of the state-of-the-art baseline methods showing efficacy of our proposed method, and 5) ablation studies showing evidences for improvement of our proposed model design.

==> takeout.tex <==
% @article{silva2014toward,
%   title={Toward embedded detection of polyps in wce images for early diagnosis of colorectal cancer},
%   author={Silva, Juan and Histace, Aymeric and Romain, Olivier and Dray, Xavier and Granado, Bertrand},
%   journal={International journal of computer assisted radiology and surgery},
%   volume={9},
%   number={2},
%   pages={283--293},
%   year={2014}
% }


% Colonoscopy is a gold standard procedure but is highly operator-dependent. Automated semantic segmentation of polyps, a precancerous precursor, can minimize missed rates and timely treatment of colorectal-related cancer at early stage. Even though there are deep learning methods steered for this task, variability in polyp size can impact model training thereby limiting it to the attribute of the majority of samples present in the training dataset that may provide sub-optimal results to a differently sized polyp. What if we exploit the size-related features in the form of text attention during training? This process can enable disentanglement of differently sized polyps already at the first few-layers of the network that will further enable feature weights at subsequent layers to adjust. Our experimental results demonstrate that such added text embedding improves overall performance of the model compared to state-of-the-art segmentation methods. In addition, our proposed  can generalize well to variable sized polyps in different datasets. We explore five different datasets and provide insights for size-specific improvements.
% Clinical motivation
% Literature basics
% Novelty of the work
% Experiments

% Ablations?
% Removing text 
% Removing layers? B2 block?
% Public datasets {Kvasir-SEG, BKAI-IGH NeoPolyp, Kvasir-Sessile, ETIS-Larib}


%All models are trained on NVIDIA GeForce RTX 3090 GPU. Before being trained, we resized all four datasets to $256 \times 256$ pixels and split them into training, validation and testing sets with a ratio of 80:10:10, except Kvasir-SEG, for which we have adopted the official split of 880/120 for training and testing respectively. We use a simple and efficient data augmentation strategy by using augmentations such as random rotation, vertical flipping, horizontal flipping, and coarse dropout. We have trained all the models on a similar configuration of hyperparameters for each dataset conisisting of Adam optimizer with a learning rate of 1e-4. We have used a batch size of 16 and an early stopping mechanism and ReduceLROnPlateau to prevent the models from overfitting.  


%Additionally, we present algorithm complexity, such as the number of trainable parameters and flops used by the methods.  

%From Table~\ref{tab:results} and Table~\ref{tganet-effect}, it can be observed that {TGANet} model consistently segment polyps with the more precise area and boundary, which shows the robustness and superiority of the proposed model. Although DeepLabV3+~\cite{chen2018encoder} and PraNet~\cite{fan2020pranet} showed the competitive results with some datasets, however, their performance were not consistent. Additionally, our method is more efficient in terms of the number of trainable parameters and flops (GMac) as compared to both DeepLabv3+~\cite{chen2018encoder} and PraNet~\cite{fan2020pranet} (see supplementary material Table 1). 
%


%The experimental results on four different datasets (including variable-sized polyps) demonstrate that our \textit{Text-guided attention network (TGANet)} is more robust and efficient as compared to other SOTA methods. %Our proposed  TGANet can generalize well to variable-sized polyps in different datasets.


% Our network can thus understand both the size-based and the number of polyp-based feature representations that contribute to feature enhancement of any underrepresented samples (e.g., small polyp size or presence of multiple polyps) that can be present. We have also used the feature enhancement module and multi-scale feature aggregation technique to further strengthen the network. 
%  for example, in most public datasets, the presence of flat or sessile polyps are lesser than obvious and large pedunculated polyps

% Q1: What are the four encoding blocks - are they different? How they have been used?  what is the difference between each block?


Medical image segmentation plays a critical role in diagnosing and treating various diseases. Accurate and efficient segmentation of medical images can help in better decision-making. However, medical image segmentation is challenging due to the complexity and variability of medical images. We propose a prototype-based approach for medical image segmentation to address these challenges. In our proposed architecture, we first learn a small initial mask of size $64\times64$ pixels. This initial mask is then used to learn the prototype for the main object label. This prototype is subsequently used to generate the final segmentation mask of size $256\times256$ pixels. By using the prototype as a representative of the object (main segmentation class), our approach handles the variability present in the medical images and helps improve the segmentation accuracy. To further improve the accuracy and robustness of the segmentation process, we introduce a prototype bank that stores and updates a fixed number of prototypes. The stored prototypes learn different features that are complementary to the object label. These features are then used together to refine the segmentation mask further. The prototype bank allows our approach to adapt to the variability of medical images and improve the segmentation accuracy across different medical datasets. In conclusion, our proposed prototype-based approach offers a promising solution for medical image segmentation. The approach is efficient, accurate, and robust and has the potential to improve clinical decision-making and patient outcomes.


shi2022ssformer



  The main contributions of the presented work include - 1) \textit{prototype learning} to generate multiple prototypes using Prototype Generation Module (PGM), which utilizes the features learned by the Pyramid Vision Transformer (PVT) encoder and the course mask generated by the Course Mask Generation Module (CMGM), 2) \textit{Course Mask Generation Module (CMGM)} uses a Large Kernel Dilated Convolution (LKDC) block, which improves the accuracy, efficiency, and generalization capabilities of the segmentation network. 3) \textit{Encoder Feature Fusion Module (EFFM)} is used to perform multi-scale feature fusion between the different features of the PVT-encoder. It utilizes factorized convolution layers and dilated convolution layers to improve its accuracy and efficiency. 4) \textit{Prototype Mask Generation Module (PMGM)} is used to generate the final prototype mask using the prototypes generated by the PGM and the output feature map of the EFFM. 5)  We have evaluated our PrototypeLab on two publicly available polyp datasets and compared it with $16$ SOTA medical image segmentation methods.

  % The main contributions of the presented work include - 1) \textit{prototype learning} to learn different features in the context of the number of polyps presence (one or many) and size (small, medium and large), 2) \textit{course mask generation module} 3) \textit{prototype Generation Module (PGM)}, 4) \textit{\ac{OoD} generalization} to strengthen the features of the encoder and pass them to the decoder. We have evaluated our PrototypeLab  on three publicly available colon polyp datasets and compared it with 18 SOTA medical image segmentation architectures. 


  \subsection{Course mask generation module}
The Course mask generation module (CMGM) generates a course mask from the feature learned by the PVT encoder. The module begins with $X_4$, where a bilinear upsampling is applied to double its spatial dimensions. The upsampled feature map is then concatenated with $X_3$ and fed into a $3\times3$ convolution layer, followed by batch normalization and ReLU activation function. After that, the module uses a novel Large Kernel Dilated Convolution (LKDC) block, which utilizes two parallel convolution layer with large kernel sizes of $7\times7$ and $13\times13$. Next, we concatenate the output of these two layers and then followed by three parallel dilated convolution layer having a dilation rate $r = \{1, 2, 4\}$. The use of the large kernels and the dilated convolutions helps to increase the receptive field which can be beneficial for capturing more contextual information and can better handle objects of varying scales. The output of the three dilated convolution layers are concatenated and then followed by a $1\times1$ convolution layer, batch normalization and ReLU activation function. The use of our Large Kernel Dilated Convolution (LKDC) block help improve its accuracy, efficiency, and generalization capabilities of the proposed segmentation network. The output from the Large Kernel Dilated Convolution (LKDC) block is again upsampled by a factor of two and then followed by a $1\times1$ convolution layer and a sigmoid activation function to generate the course mask.

\subsection{Prototype generation module}
The prototype generation module (PGM) utilize the the features from the PVT-encoder and the course mask to generate multiple different prototypes, which are later used to generate prototype masks. The module begins with use the PVT-encoder feature $X_i$, followed by $3\times3$ convolution, batch normalization and ReLU activation. Next, an element-wise multiplication is performed between the feature map and the course mask, followed by a mask average pooling to generate a feature with dimensions $B\times256\times1\times1$, here $B$ refers to the batch size. Next, we perform a mean over the batch to generate the final prototype of size $256$. In this way, we generate four different prototype $P = \{p_1, p_2, p_3, p_4\}$ from the $X_i = \{X_1, X_2, X_3, X_4\}$

After generating four prototypes, we utilize our novel Encoder Feature Fusion Module (EFFM) to perform multi-scale feature fusion between the different features of the PVT-encoder. We begin by upsampling $X_4$ by a factor of two, concatenating it with $X_3$ and then followed by $3\times3$ Conv2D-BN-ReLU. Next, again it is upsampled by a factor of two, concatenated with $X_2$ and again followed by $3\times3$ Conv2D-BN-ReLU. Similarly, we again upsample the feature map by a factor of two, concatenated with $X_1$ and again followed by $3\times3$ Conv2D-BN-ReLU. After that, we have four parallel convolution layer, where the first layer is a $1\times1$ convolution layer. In the second layer, we have factorized the $3\times3$ convolution layer to $\{3\times1\} \{1\times3\}$ layers. Similarly for rest of the two layers, we have factorized $5\times5$ and $7\times7$. Each of the three layer is then followed by a dilated convolution layer with a dilation rate $r = \{3, 5, 7\}$. The output from the first $1\times1$ convolution layer and the three dilated convolution layers are concatenated and followed by a $1\times1$ convolution layer. Now, we utilize the output feature map of the Encoder Feature Fusion Module (EFFM) to generate the final prototype $p_5$.

\subsection{Decoder}
The decoder begin by concatenating the upsampled feature map from the Course mask generation module (CMGM) with the $X_2$ and then followed by a residual block. Next again we upsample the feature map by a factor of two and then concatenate it with the $X_1$. This is then followed by a residual block. Now, we perform upsampling operation to increase the spatial dimensions by a factor of four and then concatenate it with the original input image and then followed by residual block. The output feature map would now be used to generate the prototype masks.

\subsection{Prototype mask generation module}
The Prototype Mask Generation Module (PMGM) employs cosine similarity to generate five sets of masks by comparing the output feature map of the decoder with multiple prototypes produced in the Prototype Generation Module (PGM). 

\subsection{Final mask generation}
To generate the final segmentation mask, we concatenate the output feature map of the decoder with five set of prototype masks. The concatenated feature map is then followed by a residual block and a $1\times1$ convolution and a sigmoid activation function. 

%To further improve the accuracy and robustness of the segmentation process, we introduce a prototype bank that stores and updates a fixed number of prototypes. The stored prototypes learn different features that are complementary to the object label. These features are then used together to refine the segmentation mask further. The prototype bank allows our approach to adapt to the variability of medical images and improve the segmentation accuracy across different medical datasets.



%Medical image segmentation is critical in diagnosing and treating various diseases. Accurate and efficient segmentation of medical images can help in better decision-making. However, medical image segmentation is challenging due to the complexity and variability of medical images. We propose a prototype-based approach for medical image segmentation to address these challenges. 
